Discrete representations in neural models of spoken language

The distributed and continuous representations used by neural networks are at odds with representations employed in linguistics, which are typically symbolic. Vector quantization has been proposed as a way to induce discrete neural representations that are closer in nature to their linguistic counterparts. However, it is not clear which metrics are the best-suited to analyze such discrete representations. We compare the merits of four commonly used metrics in the context of weakly supervised models of spoken language. We compare the results they show when applied to two different models, while systematically studying the effect of the placement and size of the discretization layer. We find that different evaluation regimes can give inconsistent results. While we can attribute them to the properties of the different metrics in most cases, one point of concern remains: the use of minimal pairs of phoneme triples as stimuli disadvantages larger discrete unit inventories, unlike metrics applied to complete utterances. Furthermore, while in general vector quantization induces representations that correlate with units posited in linguistics, the strength of this correlation is only moderate.

==> mean_pool.tex <==

\begin{figure}[ht]
  \centering
  \includegraphics[width=\columnwidth]{fig/meanpool.pdf}
  \caption{Pearson's $r$ RSA correlations for activations at layers
    following VQ layer with differing codebook size.  The dashed
    line shows $r$ for the equivalent layer in a model without a VQ
    layer.}
\label{fig:compare_rsa}
\end{figure}

\paragraph{Impact of discretization on phoneme encoding.} To
investigate whether learning discrete as opposed to continuous
representation results in better encoding of phonemes, we calculate
the correlation of activations of the layers following the VQ layers
with phonemes, and compare these correlations with those for the
equivalent layer in a model without a VQ
layer. Figure~\ref{fig:compare_rsa} shows these results as measured by
RSA with the cosine distance on mean-pooled activations for different
codebook sizes.

As can be seen, activations after VQ layers placed at level~1 show a
noticeably higher correlations with phonemes compared to those in a
non-VQ model, regardless of the codebook size. For VQ layers at
level~2,
only larger codebooks lead to better correlation with phonemes
compared to non-VQ activations. Activations from models with the VQ
layer placed at level~3 have consistently lower correlation with
phonemes compared to non-VQ activations. These results suggest that
discretizing visually supervised representations leads to better
encoding of phonemes at lower VQ layers, consistent with results
obtained with DC and NMI.

